Medical Reasoning in the Era of LLMs: A Systematic Review of Enhancement Techniques and Applications

The proliferation of Large Language Models (LLMs) in medicine has enabled impressive capabilities, yet a critical gap remains in their ability to perform systematic, transparent, and verifiable reasoning, a cornerstone of clinical practice. This has catalyzed a shift from single-step answer generation to the development of LLMs explicitly designed for medical reasoning. This paper provides the first systematic review of this emerging field. We propose a taxonomy of reasoning enhancement techniques, categorized into training-time strategies (e.g., supervised fine-tuning, reinforcement learning) and test-time mechanisms (e.g., prompt engineering, multi-agent systems). We analyze how these techniques are applied across different data modalities (text, image, code) and in key clinical applications such as diagnosis, education, and treatment planning. Furthermore, we survey the evolution of evaluation benchmarks from simple accuracy metrics to sophisticated assessments of reasoning quality and visual interpretability. Based on an analysis of 60 seminal studies from 2022-2025, we conclude by identifying critical challenges, including the faithfulness-plausibility gap and the need for native multimodal reasoning, and outlining future directions toward building efficient, robust, and sociotechnically responsible medical AI.

==> table1.tex <==
% 在导言区需要：
% \usepackage{booktabs}
% \usepackage{tabularx}
% \usepackage{array}

\begin{table*}[t]
\centering
\caption{A taxonomy of medical reasoning LLMs across modality, methods, applications, and evaluation.}
\label{tab:med-reasoning-taxonomy}
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{6pt}
\begin{tabularx}{\textwidth}{@{}>{\raggedright\arraybackslash}p{2.7cm} >{\raggedright\arraybackslash}p{3.2cm} X@{}}
\toprule
\textbf{Category} & \textbf{Subcategory} & \textbf{Representative works (examples)} \\
\midrule
\textbf{Modality} & Text / Code / Image &
MedReason (Wu et al., 2025c); EMULATION (Xu et al., 2024a); BP4ER (He et al., 2024); CLINICR (Nachane et al., 2024a); MedEx (Zafar et al., 2025); Med-RLVR (Zhang et al., 2025a); AlphaMed (Liu et al., 2025b); m1 (Huang et al., 2025a); FineMedLM-o1 (Yu et al., 2025a); MedAdapter (Shi et al., 2024); MC-CoT (Wei et al., 2024b); MedE2 (Mu et al., 2025); PRS-Med (Trinh et al., 2025a); AOR (Li et al., 2025e); MedAgentGym (Xu et al., 2025c); BioCoder (Tang et al., 2023); BioDSBench (Wang et al., 2024) \\
\midrule
\multirow{4}{*}{\textbf{Method — Training}} 
& Supervised Fine-Tuning &
Med-PaLM 2 (K. Singhal et al., 2023); MedTVT-R1 (Zhang et al., 2025d); HuatuoGPT-o1 (Chen et al., 2024a); EMULATION (Xu et al., 2024a); BioMed R1 (Thapa et al., 2025); MedReason (Wu et al., 2025c) \\
& Reinforcement Learning (RL) &
FineMedLM-o1 (Yu et al., 2025a); Clin-RaGen (Niu et al., 2025a); AOR (Li et al., 2025e) \\
& Multi-Stage / Chain-Aware / Position-Aware Fine-Tuning &
PRS-Med (Trinh et al., 2025a); MedGround-R1 (Xu et al., 2025a); AOR (Li et al., 2025e) \\
& RLHF / RLAIF / Structured Reward &
MedTVT-R1 (Zhang et al., 2025d); Clin-RaGen (Niu et al., 2025a); BioMed R1 (Thapa et al., 2025); MedGround-R1 (Xu et al., 2025a); AlphaMed (Liu et al., 2025c); Med-R1 (Lai et al., 2025); GMAI-VL-R1 (Su et al., 2025); HuatuoGPT-o1 (Chen et al., 2024a); Med-PaLM 2 (K. Singhal et al., 2023) \\
\midrule
\multirow{4}{*}{\textbf{Method — Reasoning}} 
& Prompt-Based Elicitation &
FineMedLM-o1 (Yu et al., 2025a); MedGround-R1 (Xu et al., 2025b); HuatuoGPT-o1 (Chen et al., 2024a); MedReason (Wu et al., 2025c); ReasonMed (Sun et al., 2025a) \\
& Selection / Aggregation &
Clinical CoT (Kwon et al., 2023); DR-CoT (Wu et al., 2024a); CoD (Chen et al., 2024c); BP4ER (He et al., 2024); MC-CoT (Wei et al., 2024b); PathCoTe (Zhou et al., 2025); O1 Replication Journey (Huang et al., 2025a,b); Self-Consistency (Wang et al., 2023a); MedAdapter (Shi et al., 2024); Ensemble Reasoning (Lucas et al., 2024) \\
& Knowledge-Enhanced Reasoning &
SelfRewardRAG (Z. Ham-mane et al., 2024); Self-BioRAG (Jeong et al., 2024); RARoK (Zhan et al., 2024); ICP (Wu et al., 2024b) \\
& Multi-Agent Systems &
MEDCO (Wei et al., 2024a); AIPatient (Yu et al., 2024); ClinicalLab (Yan et al., 2024); Agent Hospital (Li et al., 2024); AI Hospital (Fan et al., 2024); MedAgents (Tang et al., 2024); ArgMed-Agents (Hong et al., 2024); MedRAX (Fallahpour et al., 2025); ClinicalAgent (Yue et al., 2024); MedAgentGym (Xu et al., 2025c) \\
\midrule
\multirow{5}{*}{\textbf{Application}} 
& Clinical Diagnosis \& Decision Support &
DPA-GRPO (Sun et al., 2025b); AOR (Li et al., 2025e); PRS-Med (Trinh et al., 2025a); GMAI-VL-R1 (Su et al., 2025); Med-R1 (Lai et al., 2025); Med-RLVR (Zhang et al., 2025a); MedVLM-R1 (Pan et al., 2025) \\
& Medical Education \& Training & (as surveyed in figure) \\
& Medical Image Analysis \& Reasoning & (as surveyed in figure) \\
& Drug \& Molecular Discovery &
DrugAgent (Liu et al., 2025e); ChemCrow (M. Bran et al., 2024) \\
& Treatment Planning / World Models &
MedWorldModel (Yang et al., 2025); GPT-RadPlan (Liu et al., 2025d); MedRBench (Qiu et al., 2025) \\
\midrule
\multirow{3}{*}{\textbf{Evaluation / Testing}} 
& Answer Accuracy &
MedQA (Jin et al., 2020); PubMedQA (Jin et al., 2019); MedXpertQA (Zuo et al., 2025); MedAgentsBench (Tang et al., 2025); MedMCQA (Pal et al., 2022); MMLU-Clinical (Hendrycks et al., 2021) \\
& Reasoning Quality &
MedR-Bench (Qiu et al., 2025); RadRScore (Fan et al., 2025); HealthBench (Arora et al., 2025); AgentClinic (Schmidgall et al., 2024); SD-Bench (Nori et al., 2025a) \\
& Visual Interpretability &
PRS-Med (Trinh et al., 2025a); RJUA-MedDQA (Jin et al., 2024); GEMeX (Liu et al., 2024); AOR (Li et al., 2025e); GEMeX-ThinkVG (Liu et al., 2025a) \\
\bottomrule
\end{tabularx}
\end{table*}
\begin{table*}[h]
\centering
\caption{Summary of application of LLM-Agents in the medical field.}%\vspace{-2.5ex}
\renewcommand\arraystretch{1.3}
\scalebox{0.65}{
\begin{tabular}{c|cc|c|c|c}
\toprule
    % header
    \textbf{Purpose} & \multicolumn{2}{|c|}{\textbf{Functionality}} & \textbf{Work} & \textbf{Framework Type} & \textbf{Tool Use}\\
    \cline{1-6}
    % 4.1
    \multirow{10}{8em}{Clinical Decision Support and Diagnosis} & \multicolumn{2}{|c|}{Refine Diagnostic Reasoning} & \cite{dutta2024adaptivereasoningactingmedical} & Adaptive Planning & -\\
    \cline{2-6}
     & \multicolumn{2}{|c|}{Reduce Cognitive Bias} & \cite{info:doi/10.2196/59439} & Collaborative Experts & -\\
    \cline{2-6}
     & \multicolumn{2}{|c|}{Task Coordination} & \cite{wei2024medaideomnimedicalaide} & Sequential Task Chain & - \\
    \cline{2-6}
     & \multicolumn{2}{|c|}{\multirow{2}{*}{Diagnosis Accuracy}} & \cite{kim2024demonstrationadaptivecollaborationlarge} & Collaborative Experts & Yes\\ % MedRAG
    \cline{4-6}
     & && \cite{tang2024medagentslargelanguagemodels} & Collaborative Experts  & - \\
    \cline{2-6}
     & \multirow{3}{8em}{Domain Specific Functionalities} & \multicolumn{1}{|c|}{Clinical Trial Outcome Prediction} &\cite{yue2024clinicalagentclinicaltrialmultiagent} & Sequential Task Chain & Yes \\ % Section 3.3 calling additional tools
    \cline{3-6}
     & & \multicolumn{1}{|c|}{Patient Interaction Safety} & \cite{mukherjee2024polarissafetyfocusedllmconstellation} & Sequential Task Chain & - \\ % To the best of my knowledge
     %& && & \\
    \cline{3-6}
     & & \multicolumn{1}{|c|}{Prescription Validation} & \cite{van2024rxstrategistprescriptionverification} & Sequential Task Chain & Yes \\ % In the form of OCR, not sure if counts
    \cline{2-6}
     & \multicolumn{2}{|c|}{Diagnosis Capability} & \cite{yan2024clinicallabaligningagentsmultidepartmental} & Collaborative Experts & - \\
    \cline{2-6}
     & \multicolumn{2}{|c|}{Integrated Modelling} &\cite{fan2024aihospitalbenchmarkinglarge} & -- & - \\ % Not sure
    \cline{1-6}
    % 4.2
    \multirow{6}{8em}{Clinical Data Analysis and Documentation} & \multicolumn{2}{|c|}{Mortality Prediction} & \multirow{2}{*}{\cite{wang2024colacareenhancingelectronichealth}} & \multirow{2}{*}{Collaborative Experts} & \multirow{2}{*}{Yes}\\ % MSD,RAG
    \cline{2-3}
     & \multicolumn{2}{|c|}{Hospital Readmission Analysis} & & & \\
    \cline{2-6}
     & \multicolumn{2}{|c|}{Clinical Documentation} & \cite{lee2024improvingclinicaldocumentationai} & Single Agent & - \\
    \cline{2-6}
     & \multicolumn{2}{|c|}{Patient Friendly Medical Reports} & \cite{sudarshan2024agenticllmworkflowsgenerating} & Iterative Evolution & Yes \\
    \cline{2-6}
     & \multicolumn{2}{|c|}{Integrated Simulation} & \cite{li2024agenthospitalsimulacrumhospital} & Iterative Evolution & - \\
    \cline{1-6}
    % 4.3
    \multirow{6}{8em}{Medical Training and Simulation} & \multicolumn{2}{|c|}{Evaluated Diagnosis and Treatment Performance} & \cite{yan2024clinicallabaligningagentsmultidepartmental} & Collaborative Experts & - \\
    \cline{2-6}
     & \multicolumn{2}{|c|}{\multirow{2}{*}{Integrated Simulation}} & \cite{fan2024aihospitalbenchmarkinglarge} & -- & - \\
    \cline{4-6}
     & && \cite{li2024agenthospitalsimulacrumhospital} & Iterative Evolution & - \\
    \cline{2-6}
     & \multicolumn{1}{|c|}{\multirow{3}{*}{Medical Training}} & \multicolumn{1}{|c|}{\multirow{2}{*}{Training Environment}} & \cite{wei2024medcomedicaleducationcopilots} & Collaborative Experts & Yes \\
    \cline{4-6} % Order Slightly Changed for Structure Simplicity
     & & \multicolumn{1}{|c|}{} & \cite{wu2024surgboxagentdrivenoperatingroom} & Collaborative Experts & - \\
    \cline{3-6} % The multicolumn in this line fixes a bug in a not so graceful way
     & & \multicolumn{1}{|c|}{Scenario Simulation} & \cite{yu2024aipatientsimulatingpatientsehrs} & Collaborative Experts & Yes \\
    \cline{1-6}
    % 4.4
    \multirow{3}{8em}{Healthcare Service Optimization} & \multicolumn{2}{|c|}{\multirow{2}{*}{Automation of Non-diagnostic Tasks}} & \cite{mukherjee2024polarissafetyfocusedllmconstellation} & Sequential Task Chain & Yes \\
    \cline{4-6}
     & && \cite{laymouna2024roles} & -- & - \\
    \cline{2-6}
     & \multicolumn{2}{|c|}{Automation of Diagnostic Tasks} & \cite{chadebecq2023artificial} & Iterative Evolution & - \\
\bottomrule
\end{tabular}
}
\label{tab:appliction}
\end{table*}

==> table2.tex <==
\begin{table*}[htbp]
\renewcommand\arraystretch{1.2}
\centering
\caption{Common Evaluation Benchmarks and Metrics}
\scalebox{0.9}{
\begin{tabular}{c|c|l|l}
    \cline{1-4}
    \multirow{1}{*}{\textbf{Evaluation Attribute}} & \textbf{Genre} & \textbf{Specific Names} & \textbf{Related Work} \\
    \cline{1-4}
    \multirow{11}{*}{Benchmarks} & \multirow{5}{10em}{Static Q\&A Benchmarks} & \textit{MedQA} & \cite{jin2020diseasedoespatienthave} \\
    \cline{3-4}
     & & \textit{MedMCQA} & \cite{pmlr-v174-pal22a} \\
    \cline{3-4}
     & & \textit{Pub-MedQA} & \cite{jin2019pubmedqa} \\
    \cline{3-4}
     & & \multirow{2}{*}{\textit{MMLU}} & \cite{hendryckstest2021} \\
    % \cline{4-4} % Looks better without --ayu
     & & & \cite{hendrycks2021ethics} \\
    \cline{2-4}
     & \multirow{4}{10em}{Workflow-Based Simulation Benchmarks} & \textit{MedChain} & \cite{liu2024medchainbridginggapllm} \\
    \cline{3-4}
     & & \textit{AI Hospital} & \cite{fan2024aihospitalbenchmarkinglarge} \\
    \cline{3-4}
     & & \textit{AgentClinic} & \cite{schmidgall2024agentclinic} \\
    \cline{3-4}
     & & \textit{ClinicalLab} & \cite{yan2024clinicallabaligningagentsmultidepartmental} \\
    \cline{2-4}
     & \multirow{2}{10em}{Automated Evaluation Frameworks} & \textit{AI-SCE} & \cite{Mehandru2024EvaluatingLL} \\
    \cline{3-4}
     & & \textit{RJUA-SPs} & \cite{10.1145/3637528.3671575} \\ % Best citation key ever! --ayu
    \cline{1-4}
    \multirow{9}{7em}{Metrics for Task-Specific Evaluation} & \multirow{3}{10em}{Exact Match Metrics} & Accuracy & -- \\
    \cline{3-4}
     & & Precision & -- \\
    \cline{3-4}
     & & Recall & -- \\
    \cline{2-4}
     & \multirow{3}{10em}{Semantic Similarity Metrics} & \textbf{BLEU} & \cite{papineni-etal-2002-bleu} \\
    \cline{3-4}
     & & \textbf{ROUGE} & \cite{lin-2004-rouge} \\
    \cline{3-4}
     & & \textbf{BertScore} & \cite{zhang2020bertscoreevaluatingtextgeneration} \\
    \cline{2-4}
     & \multirow{3}{10em}{LLM-Based Evaluation Metrics} & \textit{ChatCoach} & \cite{huang2024benchmarkinglargelanguagemodels} \\
    \cline{3-4}
     & & \multirow{2}{10em}{Retrival-Augmented Evaluation Framework} & \multirow{2}{*}{\cite{10.1145/3637528.3671575}} \\ % Lazy Formatting --ayu
    &&&\\
    \cline{1-4}
\end{tabular}
}
% \vspace{-2.5ex}
\label{tab:eval}
\end{table*}

==> table3.tex <==
% 在导言区需要：

% \usepackage{booktabs}
% \usepackage{tabularx}
% \usepackage{array}

\begin{table*}[t]
\centering
\caption{A taxonomy of medical reasoning LLMs across modality, methods, applications, and evaluation.}
\label{tab:med-reasoning-taxonomy}
\renewcommand{\arraystretch}{1.15}
\setlength{\tabcolsep}{6pt}
\begin{tabularx}{\textwidth}{@{}>{\raggedright\arraybackslash}p{2.7cm} >{\raggedright\arraybackslash}p{3.2cm} X@{}}
\toprule
\textbf{Category} & \textbf{Subcategory} & \textbf{Representative works (examples)} \\
\midrule
\textbf{Modality} & Text / Code / Image &
MedReason (Wu et al., 2025c); EMULATION (Xu et al., 2024a); BP4ER (He et al., 2024); CLINICR (Nachane et al., 2024a); MedEx (Zafar et al., 2025); Med-RLVR (Zhang et al., 2025a); AlphaMed (Liu et al., 2025b); m1 (Huang et al., 2025a); FineMedLM-o1 (Yu et al., 2025a); MedAdapter (Shi et al., 2024); MC-CoT (Wei et al., 2024b); MedE2 (Mu et al., 2025); PRS-Med (Trinh et al., 2025a); AOR (Li et al., 2025e); MedAgentGym (Xu et al., 2025c); BioCoder (Tang et al., 2023); BioDSBench (Wang et al., 2024) \\
\midrule
\multirow{4}{*}{\textbf{Method — Training}} 
& Supervised Fine-Tuning &
Med-PaLM 2 (K. Singhal et al., 2023); MedTVT-R1 (Zhang et al., 2025d); HuatuoGPT-o1 (Chen et al., 2024a); EMULATION (Xu et al., 2024a); BioMed R1 (Thapa et al., 2025); MedReason (Wu et al., 2025c) \\
& Reinforcement Learning (RL) &
FineMedLM-o1 (Yu et al., 2025a); Clin-RaGen (Niu et al., 2025a); AOR (Li et al., 2025e) \\
& Multi-Stage / Chain-Aware / Position-Aware Fine-Tuning &
PRS-Med (Trinh et al., 2025a); MedGround-R1 (Xu et al., 2025a); AOR (Li et al., 2025e) \\
& RLHF / RLAIF / Structured Reward &
MedTVT-R1 (Zhang et al., 2025d); Clin-RaGen (Niu et al., 2025a); BioMed R1 (Thapa et al., 2025); MedGround-R1 (Xu et al., 2025a); AlphaMed (Liu et al., 2025c); Med-R1 (Lai et al., 2025); GMAI-VL-R1 (Su et al., 2025); HuatuoGPT-o1 (Chen et al., 2024a); Med-PaLM 2 (K. Singhal et al., 2023) \\
\midrule
\multirow{4}{*}{\textbf{Method — Reasoning}} 
& Prompt-Based Elicitation &
FineMedLM-o1 (Yu et al., 2025a); MedGround-R1 (Xu et al., 2025b); HuatuoGPT-o1 (Chen et al., 2024a); MedReason (Wu et al., 2025c); ReasonMed (Sun et al., 2025a) \\
& Selection / Aggregation &
Clinical CoT (Kwon et al., 2023); DR-CoT (Wu et al., 2024a); CoD (Chen et al., 2024c); BP4ER (He et al., 2024); MC-CoT (Wei et al., 2024b); PathCoTe (Zhou et al., 2025); O1 Replication Journey (Huang et al., 2025a,b); Self-Consistency (Wang et al., 2023a); MedAdapter (Shi et al., 2024); Ensemble Reasoning (Lucas et al., 2024) \\
& Knowledge-Enhanced Reasoning &
SelfRewardRAG (Z. Ham-mane et al., 2024); Self-BioRAG (Jeong et al., 2024); RARoK (Zhan et al., 2024); ICP (Wu et al., 2024b) \\
& Multi-Agent Systems &
MEDCO (Wei et al., 2024a); AIPatient (Yu et al., 2024); ClinicalLab (Yan et al., 2024); Agent Hospital (Li et al., 2024); AI Hospital (Fan et al., 2024); MedAgents (Tang et al., 2024); ArgMed-Agents (Hong et al., 2024); MedRAX (Fallahpour et al., 2025); ClinicalAgent (Yue et al., 2024); MedAgentGym (Xu et al., 2025c) \\
\midrule
\multirow{5}{*}{\textbf{Application}} 
& Clinical Diagnosis \& Decision Support &
DPA-GRPO (Sun et al., 2025b); AOR (Li et al., 2025e); PRS-Med (Trinh et al., 2025a); GMAI-VL-R1 (Su et al., 2025); Med-R1 (Lai et al., 2025); Med-RLVR (Zhang et al., 2025a); MedVLM-R1 (Pan et al., 2025) \\
& Medical Education \& Training & (as surveyed in figure) \\
& Medical Image Analysis \& Reasoning & (as surveyed in figure) \\
& Drug \& Molecular Discovery &
DrugAgent (Liu et al., 2025e); ChemCrow (M. Bran et al., 2024) \\
& Treatment Planning / World Models &
MedWorldModel (Yang et al., 2025); GPT-RadPlan (Liu et al., 2025d); MedRBench (Qiu et al., 2025) \\
\midrule
\multirow{3}{*}{\textbf{Evaluation / Testing}} 
& Answer Accuracy &
MedQA (Jin et al., 2020); PubMedQA (Jin et al., 2019); MedXpertQA (Zuo et al., 2025); MedAgentsBench (Tang et al., 2025); MedMCQA (Pal et al., 2022); MMLU-Clinical (Hendrycks et al., 2021) \\
& Reasoning Quality &
MedR-Bench (Qiu et al., 2025); RadRScore (Fan et al., 2025); HealthBench (Arora et al., 2025); AgentClinic (Schmidgall et al., 2024); SD-Bench (Nori et al., 2025a) \\
& Visual Interpretability &
PRS-Med (Trinh et al., 2025a); RJUA-MedDQA (Jin et al., 2024); GEMeX (Liu et al., 2024); AOR (Li et al., 2025e); GEMeX-ThinkVG (Liu et al., 2025a) \\
\bottomrule
\end{tabularx}
\end{table*}

